Losing Confidence in Quality: Unspoken Evolution of Computer Vision Services

Recent advances in artificial intelligence (AI) and machine learning (ML), such as computer vision, are now available as intelligent services and their accessibility and simplicity is compelling. Multiple vendors now offer this technology as cloud services and developers want to leverage these advances to provide value to end-users. However, there is no firm investigation into the maintenance and evolution risks arising from use of these intelligent services; in particular, their behavioural consistency and transparency of their functionality. We evaluated the responses of three different intelligent services (specifically computer vision) over 11 months using 3 different data sets, verifying responses against the respective documentation and assessing evolution risk. We found that there are: (1) inconsistencies in how these services behave; (2) evolution risk in the responses; and (3) a lack of clear communication that documents these risks and inconsistencies. We propose a set of recommendations to both developers and intelligent service providers to inform risk and assist maintainability.

==> preamble/simple.tex <==
\usepackage{hyperref}
\input{simple/author}
\input{simple/captions}
\input{simple/cleverref}
\input{simple/geometry}
\input{simple/graphics}
\input{simple/typesetting}

==> preamble/simple/author.tex <==
\author{Alex Cummaudo\\Applied Artificial Intelligence Institute\\Deakin University, Australia}
\date{\today}


==> preamble/simple/captions.tex <==
\usepackage[labelfont=bf]{caption}

==> preamble/simple/cleverref.tex <==
\usepackage[capitalise,noabbrev,nameinlink]{cleveref}
\Crefname{lstlisting}{Listing}{Listings}

==> preamble/simple/geometry.tex <==
\usepackage{geometry}
\newgeometry{top=2.25cm,right=2cm,bottom=2.5cm,left=3cm}


==> preamble/simple/graphics.tex <==
\usepackage{graphicx}
\graphicspath{{images/}{../images/}}


==> preamble/simple/typesetting.tex <==
% Linespread of 1.5 as required by SIT
\linespread{1.5}
% Times new roman package
\usepackage{mathptmx}
% Change font style for sub-sub section
\usepackage{sectsty}
\subsubsectionfont{\normalfont\itshape}
